Mirror-3DGS: Incorporating Mirror Reflections into 3D Gaussian Splatting

3D Gaussian Splatting (3DGS) has significantly advanced 3D scene reconstruction and novel view synthesis. However, like Neural Radiance Fields (NeRF), 3DGS struggles with accurately modeling physical reflections, particularly in mirrors, leading to incorrect reconstructions and inconsistent reflective properties. To address this challenge, we introduce Mirror-3DGS, a novel framework designed to accurately handle mirror geometries and reflections, thereby generating realistic mirror reflections. By incorporating mirror attributes into 3DGS and leveraging plane mirror imaging principles, Mirror-3DGS simulates a mirrored viewpoint from behind the mirror, enhancing the realism of scene renderings. Extensive evaluations on both synthetic and real-world scenes demonstrate that our method can render novel views with improved fidelity in real-time, surpassing the state-of-the-art Mirror-NeRF, especially in mirror regions.

==> figure/converge_qualitative.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{file/converge_qualitative.pdf}
\vskip -0.2in
\caption{
 \textbf{Evolution of rendering results over training time on the washroom scene.} Our Mirror-3DGS rapidly learns to accurately render contents in mirrors, while Mirror-NeRF takes more than five hours to reach similar levels of detail.
} 
\label{figure:converge_qualitative}
\vskip -0.2in
\end{figure}

==> figure/converge_quantitative.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{file/converge_quantitative.pdf}
\caption{
Convergence speed comparison on the washroom scene. Our method achieves optimal rendering results in approximately 15 minutes, significantly outpacing Mirror-NeRF, which requires over 8 hours to reach a comparable level of performance.
} 
\label{figure:converge_quantitative}
\vskip -0.2in
\end{figure}

==> table/ablation_market.tex <==
\setlength{\tabcolsep}{13.0pt}{
\begin{table}[tb]
   \caption{
   Ablation results on the challenging test set of real market scene. The values in red parentheses indicate metric changes relative to our full method.
   }
  \label{table:ablation_market}
  \centering
  \begin{tabular}{lccc}
    \toprule
    & PSNR↑ & SSIM↑ & LPIPS↓ \\
    \midrule
    w/o $\mathcal{L}_{mask}$ & 25.68 \textcolor{red}{(↓1.50)}& 0.83 \textcolor{red}{(↓0.01)} & 0.05 \textcolor{red}{(↑0.01)}\\
    w/o $\mathcal{L}_{depth}$ & 25.39 \textcolor{red}{(↓1.79)}& 0.82 \textcolor{red}{(↓0.02)}& 0.05 \textcolor{red}{(↑0.01)}\\
    w/o $\mathcal{L}_{plane}$ & 26.84 \textcolor{red}{(↓0.34)}& 0.84 \textcolor{red}{\phantom{(↓0.00)}}& 0.04 \textcolor{red}{\phantom{(↑0.00)}}\\
    \midrule
    \textbf{Our full method} & 27.18 \textcolor{red}{\phantom{(↓0.00)}}& 0.84 \textcolor{red}{\phantom{(↓0.00)}}& 0.04 \textcolor{red}{\phantom{(↑0.00)}}\\
    \bottomrule
  \end{tabular}
\end{table}
}

==> table/ablation_washroom.tex <==
\setlength{\tabcolsep}{13.0pt}{
\begin{table}[!tb]
   \caption{
   Ablation results on the challenging test set of synthetic washroom scene. The values in red parentheses indicate metric changes relative to our full method.
   }
  \label{table:ablation_washroom}
  \centering
  \begin{tabular}{lccc}
    \toprule
    & PSNR↑ & SSIM↑ & LPIPS↓ \\
    \midrule
    w/o $\mathcal{L}_{mask}$ & 17.27 \textcolor{red}{(↓3.03)}& 0.69 \textcolor{red}{(↓0.06)}& 0.13 \textcolor{red}{(↑0.04)}\\
    w/o $\mathcal{L}_{depth}$ & 18.61 \textcolor{red}{(↓1.69)}& 0.72 \textcolor{red}{(↓0.03)}& 0.11 \textcolor{red}{(↑0.02)}\\
    
    w/o $\mathcal{L}_{plane}$ & 16.29 \textcolor{red}{(↓4.01)}& 0.67 \textcolor{red}{(↓0.08)}& 0.15 \textcolor{red}{(↑0.06)}\\
    \midrule
    \textbf{Our full method} & 20.30 \textcolor{red}{\phantom{(↓0.00)}}& 0.75 \textcolor{red}{\phantom{(↓0.00)}}& 0.09 \textcolor{red}{\phantom{(↑0.00)}}\\
    \bottomrule
  \end{tabular}
\end{table}
}


==> table/challenging_test.tex <==
\setlength{\tabcolsep}{0.1pt}{
\begin{table}[tb]
   \caption{Quantitative comparison on the \textbf{challenging test set} with all images containing mirrors. Best results are \textbf{bolded} and second best are \underline{underlined}. Methods marked with `*' are evaluated only on mirror regions.}
  \label{table:challending_test_comparison}
  \centering
  \scriptsize
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{2.5}{*}{Method} & \multicolumn{4}{c}{Synthetic} && \multicolumn{4}{c}{Real} \\
    \cmidrule{2-5} \cmidrule{7-10}
    & PSNR↑ & SSIM↑ & LPIPS↓ & FPS↑ && PSNR↑ & SSIM↑ & LPIPS↓  & FPS↑\\
    \cmidrule{2-5} \cmidrule{7-10}
    InstantNGP~\cite{muller2022instant} & 14.26 & 0.44 & 0.65 & 9.22 && 10.54 & 0.20 & 0.72 & 13.00 \\
    \cmidrule{2-5} \cmidrule{7-10}
    DVGO~\cite{sun2022direct} & 17.65 & 0.63 & 0.49 & 4.34 && 22.28 & 0.68 & 0.32& 4.41 \\
    \cmidrule{2-5} \cmidrule{7-10}
    Mirror-NeRF~\cite{zeng2023mirror} & \textbf{27.33} & \textbf{0.94} & \textbf{0.05} & 0.55 && \textbf{25.25} & \textbf{0.86} & \textbf{0.06} & 0.55\\
    \midrule
    \midrule
    3DGS~\cite{3dgs} & 22.15 & 0.84 & 0.17 & \textbf{275.73}  && 22.13 & 0.72 & 0.24 & \textbf{208.23} \\
    \cmidrule{2-5} \cmidrule{7-10}
    Evoluted-3DGS & 21.82 & 0.82 & 0.09 & \underline{195.36} && 21.59 & 0.75 & 0.11 & \underline{98.49}\\
    \cmidrule{2-5} \cmidrule{7-10}
    \textbf{Mirror-3DGS (Ours)} & \underline{24.73} & \underline{0.85} & \underline{0.06} & 120.61 && \underline{23.01} & \underline{0.77} & \underline{0.09} & 95.22 \\
    \midrule
    \midrule
    3DGS*~\cite{3dgs} & 16.42 & - & - & - && 21.27 & - & - & -\\
    Mirror-NeRF*~\cite{zeng2023mirror} & \textcolor{blue}{\textbf{22.14}} & - & - & - && 22.18 & - & - & -\\
    \textbf{Mirror-3DGS* (Ours)} & 21.60 & - & - & - && \textcolor{blue}{\textbf{22.94}} & - & - & - \\
    \bottomrule
  \end{tabular}
\end{table}
}

